Learning and Policy Search in Stochastic Dynamical Systems with Bayesian Neural Networks

We present an algorithm for model-based reinforcement learning that combines Bayesian neural networks (BNNs) with random roll-outs and stochastic optimization for policy learning. The BNNs are trained by minimizing $\alpha$-divergences, allowing us to capture complicated statistical patterns in the transition dynamics, e.g. multi-modality and heteroskedasticity, which are usually missed by other common modeling approaches. We illustrate the performance of our method by solving a challenging benchmark where model-based approaches usually fail and by obtaining promising results in a real-world scenario for controlling a gas turbine.

==> comparison_gps.tex <==

\newcommand{\ica}{\hspace{0.25cm}}

\renewcommand{\arraystretch}{0.94}

\subsection{Comparison with Gaussian processes}

%Gaussian processes (GPs) are another probabilistic approach for modeling
%dynamics in reinforcement learning algorithms
%5\cite{Rasmussen2004,ko2007gaussian}. These methods have been very successful at
%5model-based policy learning in the scarce data regime
%\cite{deisenroth2011pilco}. However, our proposed approach based on
%probabilistic neural networks (NNs) trained by minimizing $\alpha$-divergences
%have several advantages over GPs in the large data regime. The first one is
%computational. NNs have better scalability properties than GPs and by using
%GPUs you can apply these methods to very large datasets. The second advantage
%is statistical. In section, \ref{sec:toy_problems} we have shown that our
%probabilistic NNs are very flexible models with predictive distributions that
%can capture complicated patterns such as bi-modality and heteroskedasticity.
%GPs are based on homoskedastic Gaussian prior distributions that cannot capture
%such patterns.

We now compare the predictions of Bayesian networks (BNNs) with $\alpha=0.5$
with those of Gaussian processes (GPs). We considered the data for the
Wet-Chicken and Turbine problems. We split the available data into training
and test sets with 75\% and 25\% of the data. For scalability, we used sparse
GPs based on the FITC approximation \cite{snelson2005sparse}, using a total of
150 inducing points. Table \ref{tab:gps} shows the average test RMSE for each
method. Overall, BBNs with $\alpha = 0.5$ obtain higher test log-likelihood,
which shows that they are better at capturing the statistical properties of the
true dynamics.


\begin{wraptable}{t}{6.5cm}
%\begin{table}
\begin{center}
\vspace{-1.5cm}
\caption{Comparison with Gaussian processes}
\label{tab:gps}
\resizebox{0.425\textwidth}{!}{
\begin{tabular}{@{\ica}l@{\ica}c@{\ica}c@{\ica}c@{\ica}c@{\ica}}
\toprule
& \multicolumn{2}{c}{\bf Wet-Chicken } & \multicolumn{2}{c}{\bf Turbine } \\
\midrule
{\bf Method} & RMSE & LL & RMSE & LL \\
\midrule
$\alpha = 0.5$ & 1.19 & {\bf -0.05} & {\bf 0.30 } & {\bf 0.71}\\
Sparse GP & {\bf 1.15 } & -1.73 & 0.32 & 0.45\\
\bottomrule
\end{tabular}
}
\end{center}
%\end{table}
\end{wraptable}



